Exozodiacal clouds: Hot and warm dust around main sequence stars

A warm/hot dust component (at temperature $>$ 300K) has been detected around $\sim$ 20% of stars. This component is called "exozodiacal dust" as it presents similarities with the zodiacal dust detected in our Solar System, even though its physical properties and spatial distribution can be significantly different. Understanding the origin and evolution of this dust is of crucial importance, not only because its presence could hamper future detections of Earth-like planets in their habitable zones, but also because it can provide invaluable information about the inner regions of planetary systems. In this review, we present a detailed overview of the observational techniques used in the detection and characterisation of exozodiacal dust clouds ("exozodis") and the results they have yielded so far, in particular regarding the incidence rate of exozodis as a function of crucial parameters such as stellar type and age, or the presence of an outer cold debris disc. We also present the important constraints that have been obtained, on dust size distribution and spatial location, by using state-of-the-art radiation transfer models on some of these systems. Finally, we investigate the crucial issue of how to explain the presence of exozodiacal dust around so many stars (regardless of their ages) despite the fact that such dust so close to its host star should disappear rapidly due to the coupled effect of collisions and stellar radiation pressure. Several potential mechanisms have been proposed to solve this paradox and are reviewed in detail in this paper. The review finishes by presenting the future of this growing field.

==> journals_short.tex <==
\newcommand{\AAp}      {Astron. Astrophys.}
\newcommand{\AApR}     {Astron. Astrophys. Rev.}
\newcommand{\AApS}    {AApS}
\newcommand{\AApSS}    {AApSS}
\newcommand{\AApT}     {Astron. Astrophys. Trans.}
\newcommand{\AdvSR}    {Adv. Space Res.}
\newcommand{\AJ}       {Astron. J.}
\newcommand{\AN}       {Astron. Nachr.}
\newcommand{\AO}       {App. Optics}
\newcommand{\ApJ}      {Astrophys. J.}
\newcommand{\ApJL}      {Astrophys. J. Lett.}
\newcommand{\ApJS}     {Astrophys. J. Suppl.}
\newcommand{\ApSS}     {Astrophys. Space Sci.}
\newcommand{\ARAA}     {Ann. Rev. Astron. Astrophys.}
\newcommand{\ARevEPS}  {Ann. Rev. Earth Planet. Sci.}
\newcommand{\BAAS}     {BAAS}
\newcommand{\CelMech}  {Celest. Mech. Dynam. Astron.}
\newcommand{\EMP}      {Earth, Moon and Planets}
\newcommand{\EPS}      {Earth, Planets and Space}
\newcommand{\GRL}      {Geophys. Res. Lett.}
\newcommand{\JGR}      {J. Geophys. Res.}
\newcommand{\JOSAA}    {J. Opt. Soc. Am. A}
\newcommand{\MemSAI}   {Mem. Societa Astronomica Italiana}
\newcommand{\MNRAS}    {MNRAS}
\newcommand{\PASJ}     {PASJ}
\newcommand{\PASP}     {PASP}
\newcommand{\PSS}      {Planet. Space Sci.}
\newcommand{\QJRAS}    {Quart. J. Roy. Astron. Soc.}
\newcommand{\RAA}      {Research in Astron. Astrophys.}
\newcommand{\SolPhys}  {Sol. Phys.}
\newcommand{\SolSysRes}{Sol. Sys. Res.}
\newcommand{\SSR}      {Space Sci. Rev.}

\endinput

   TeX macro    Journal name
   ---------    ---------------------------------------------------------
   aj           Astronomical Journal
   araa         Annual Review of Astron and Astrophys
   apj          Astrophysical Journal
   apjl         Astrophysical Journal, Letters
   apjs         Astrophysical Journal, Supplement
   ao           Applied Optics
   apss         Astrophysics and Space Science
   aap          Astronomy and Astrophysics
   aapr         Astronomy and Astrophysics Reviews
   aaps         Astronomy and Astrophysics, Supplement
   azh          Astronomicheskii Zhurnal
   baas         Bulletin of the AAS
   jrasc        Journal of the RAS of Canada
   memras       Memoirs of the RAS
   mnras        Monthly Notices of the RAS
   pra          Physical Review A: General Physics
   prb          Physical Review B: Solid State
   prc          Physical Review C
   prd          Physical Review D
   pre          Physical Review E
   prl          Physical Review Letters
   pasp         Publications of the ASP
   pasj         Publications of the ASJ
   qjras        Quarterly Journal of the RAS
   skytel       Sky and Telescope
   solphys      Solar Physics
   sovast       Soviet Astronomy
   ssr          Space Science Reviews
   zap          Zeitschrift fuer Astrophysik
   nat          Nature
   iaucirc      IAU Cirulars
   aplett       Astrophysics Letters
   apspr        Astrophysics Space Physics Research
   bain         Bulletin Astronomical Institute of the Netherlands
   fcp          Fundamental Cosmic Physics
   gca          Geochimica Cosmochimica Acta
   grl          Geophysics Research Letters
   jcp          Journal of Chemical Physics
   jgr          Journal of Geophysics Research
   jqsrt        Journal of Quantitiative Spectroscopy and Radiative Trasfer
   memsai       Mem. Societa Astronomica Italiana
   nphysa       Nuclear Physics A
   physrep      Physics Reports
   physscr      Physica Scripta
   planss       Planetary Space Science
   procspie     Proceedings of the SPIE


